Self-adjusting Advertisement of Cache Indicators with Bandwidth Constraints

Cache advertisements reduce the access cost by allowing users to skip the cache when it does not contain their datum. Such advertisements are used in multiple networked domains such as 5G networks, wide area networks, and information-centric networking. The selection of an advertisement strategy exposes a trade-off between the access cost and bandwidth consumption. Still, existing works mostly apply a trial-and-error approach for selecting the best strategy, as the rigorous foundations required for optimizing such decisions is lacking. Our work shows that the desired advertisement policy depends on numerous parameters such as the cache policy, the workload, the cache size, and the available bandwidth. In particular, we show that there is no ideal single configuration. Therefore, we design an adaptive, self-adjusting algorithm that periodically selects an advertisement policy. Our algorithm does not require any prior information about the cache policy, cache size, or workload, and does not require any apriori configuration. Through extensive simulations, using several state-of-the-art cache policies, and real workloads, we show that our approach attains a similar cost to that of the best static configuration (which is only identified in retrospect) in each case.

==> Figs/FnFpByUpdateInterval_only_16bpe.tex <==
    \begin{tikzpicture}
        log bases x={2},
        log bases y={10},
        \begin{groupplot}[
            group style=
                {
                columns=2,
                xlabels at=edge bottom,
                ylabels at=edge left,
                horizontal sep=0.07\columnwidth,
                group name=plots
                },
    		width  = 0.55*\columnwidth,
     		height = 0.4*\columnwidth,
    		xmode = log,
    		ymode = log,
    		xmin = 2,
     		xmax = 8192,
     		xtick = {2, 16, 128, 1024, 8192},
     		xticklabels = {2,16,128,1K,8K},
     		ymin = 0.0001,
     		ymax = 0.3,
     		ytick = {0.0001,0.001,0.01,0.1},
     		minor tick style={draw=none},
      		yticklabels = {$10^{-4}$,$10^{-3}$,$10^{-2}$, $10^{-1}$},
            ymajorgrids = true,
            ylabel = {Ratio},
     		ylabel near ticks,
    		legend style = {at={(-0.1,1.65)},anchor=north,legend columns=-1,font=\footnotesize},
    		xlabel = {Update interval (\#requests)}, 
    		xlabel near ticks,
    	    label style={font=\footnotesize},
    	    tick label style={font=\footnotesize},
    	]
        	
        \nextgroupplot[
            title = False negative,
            title style ={
                font=\footnotesize,
                yshift = -2pt
                },
     		]

            \addplot[color=purple, mark=+, 				width = \plotwidth] coordinates {
            (1.0000, 0.0001)(2.0000, 0.0002)(4.0000, 0.0003)(8.0000, 0.0012)(16.0000, 0.0077)(32.0000, 0.0216)(64.0000, 0.0376)(128.0000, 0.0513)(256.0000, 0.0655)(512.0000, 0.0818)(1024.0000, 0.1028)(2048.0000, 0.1289)(4096.0000, 0.1602)(8192.0000, 0.1869)
            };

        
        \nextgroupplot[
            title = False positive,
            title style ={
                font=\footnotesize,
                yshift = -2pt,
                },
      		yticklabels = \empty
      	]

            \addplot[color=purple, mark=+, 				width = \plotwidth] coordinates {
            (1.0000, 0.0003)(2.0000, 0.0003)(4.0000, 0.0003)(8.0000, 0.0003)(16.0000, 0.0003)(32.0000, 0.0003)(64.0000, 0.0004)(128.0000, 0.0005)(256.0000, 0.0007)(512.0000, 0.0011)(1024.0000, 0.0018)(2048.0000, 0.0032)(4096.0000, 0.0061)(8192.0000, 0.0116)
            };\addlegendentry {16-BPE}
        \end{groupplot}3 
    \end{tikzpicture}


==> Figs/costByIndSize.tex <==
%\resizebox{\columnwidth}{0.5\columnwidth}{
\renewcommand{\xmin}{1}
\renewcommand{\xmax}{13}
\begin{figure}[ht]
    \subfloat [ C1K Lru $\missp = 3$ Scarab] { 
        \begin{tikzpicture}
        	\begin{axis}[
        		width  = \plotwidth,
         		height = \plotheight,
        		xmin = \xmin,
        		xmax = \xmax,
        		legend style = {at={(0.5,1.23)},anchor=north,legend columns=-1,font=\footnotesize},
        		ylabel = Service Cost,
         		ylabel near ticks,
        		xlabel = {Indicator Size [bits per element]},
        		xlabel near ticks,
        	    label style={font=\footnotesize},
        	    tick label style={font=\footnotesize},
        	]
            \addplot[color=black, mark=triangle, width = \plotwidth] coordinates {
                (2.0000, 2.7475)(2.4000, 2.7989)(2.8800, 2.7792)(3.4550, 2.7304)(4.1470, 2.7134)(4.9760, 2.6964)(5.9710, 2.6828)(7.1660, 2.6893)(8.5990, 2.6929)(10.3190, 2.7046)(12.3830, 2.7176)(14.8600, 2.7337)(17.8320, 2.7417)(21.3980, 2.7578)(25.6780, 2.7618)(30.8140, 2.7729)(36.9760, 2.7779)
            };  \addlegendentry {$B$ = 10}
            
            \addplot[color=red, mark=o, width = \plotwidth] coordinates {
                (2.0000, 2.7475)(2.4000, 2.7086)(2.8800, 2.6751)(3.4550, 2.6020)(4.1470, 2.5675)(4.9760, 2.6252)(5.9710, 2.6220)(7.1660, 2.6177)(8.5990, 2.6185)(10.3190, 2.6254)(12.3830, 2.6331)(14.8600, 2.6455)(17.8320, 2.6531)(21.3980, 2.6723)(25.6780, 2.6842)(30.8140, 2.7012)(36.9760, 2.7164)
            };  \addlegendentry {$B$ = 30}
            
            \addplot[color=blue, mark=x, width = \plotwidth]    coordinates {
                (2.0000, 2.7475)(2.4000, 2.7086)(2.8800, 2.6751)(3.4550, 2.6020)(4.1470, 2.5675)(4.9760, 2.5287)(5.9710, 2.5023)(7.1660, 2.4854)(8.5990, 2.5871)(10.3190, 2.5923)(12.3830, 2.5993)(14.8600, 2.6092)(17.8320, 2.6214)(21.3980, 2.6316)(25.6780, 2.6449)(30.8140, 2.6530)(36.9760, 2.6722)
            };  \addlegendentry {$B$ = 50}

        \end{axis}
        \end{tikzpicture}
    }
    
        \subfloat [ C=1000 Lfu $\missp = 3$ Scarab] { 
        \begin{tikzpicture}
        	\begin{axis}[
        		width  = \plotwidth,
         		height = \plotheight,
        		xmin = \xmin,
        		xmax = \xmax,
        		legend style = {at={(0.5,1.23)},anchor=north,legend columns=-1,font=\footnotesize},
        		ylabel = Service Cost,
         		ylabel near ticks,
        		xlabel = {Indicator Size [bits per element]},
        		xlabel near ticks,
        	    label style={font=\footnotesize},
        	    tick label style={font=\footnotesize},
        	]
            \addplot[color=black, mark=triangle, width = \plotwidth] coordinates {
                (2.0000, 2.6139)(2.4000, 2.5945)(2.8800, 2.5668)(3.4550, 2.5105)(4.1470, 2.4815)(4.9760, 2.4532)(5.9710, 2.4300)(7.1660, 2.4155)(8.5990, 2.4075)(10.3190, 2.4033)(12.3830, 2.4018)(14.8600, 2.4028)(17.8320, 2.4058)(21.3980, 2.4092)(25.6780, 2.4141)(30.8140, 2.4169)(36.9760, 2.4218)
            };  \addlegendentry {$B$ = 10}
            
            \addplot[color=red, mark=o, width = \plotwidth] coordinates {
                (2.0000, 2.6139)(2.4000, 2.5785)(2.8800, 2.5472)(3.4550, 2.4789)(4.1470, 2.4463)(4.9760, 2.4129)(5.9710, 2.4170)(7.1660, 2.4036)(8.5990, 2.3981)(10.3190, 2.3942)(12.3830, 2.3929)(14.8600, 2.3942)(17.8320, 2.3951)(21.3980, 2.3961)(25.6780, 2.3976)(30.8140, 2.3987)(36.9760, 2.4023)
            };  \addlegendentry {$B$ = 30}
            
            \addplot[color=blue, mark=x, width = \plotwidth]    coordinates {
                (2.0000, 2.6139)(2.4000, 2.5785)(2.8800, 2.5472)(3.4550, 2.4789)(4.1470, 2.4463)(4.9760, 2.4129)(5.9710, 2.3871)(7.1660, 2.3704)(8.5990, 2.3833)(10.3190, 2.3874)(12.3830, 2.3871)(14.8600, 2.3883)(17.8320, 2.3914)(21.3980, 2.3927)(25.6780, 2.3937)(30.8140, 2.3950)(36.9760, 2.3972)
            };  \addlegendentry {$B$ = 50}
            
        \end{axis}
        \end{tikzpicture}
    }
    
    \subfloat [ C1K Lru $\missp = 10$ Scarab] { 
        \begin{tikzpicture}
        	\begin{axis}[
        		width  = \plotwidth,
         		height = \plotheight,
        		xmin = \xmin,
        		xmax = \xmax,
        		legend style = {at={(0.5,1.23)},anchor=north,legend columns=-1,font=\footnotesize},
        		ylabel = Service Cost,
         		ylabel near ticks,
        		xlabel = {Indicator Size [bits per element]},
        		xlabel near ticks,
        	    label style={font=\footnotesize},
        	    tick label style={font=\footnotesize},
        	]
        \addplot[color=black, mark=triangle, width = \plotwidth] coordinates {
            (2.0000, 7.8602)(2.4000, 8.2131)(2.8800, 8.2384)(3.4550, 8.2687)(4.1470, 8.3045)(4.9760, 8.3542)(5.9710, 8.3786)(7.1660, 8.4543)(8.5990, 8.5015)(10.3190, 8.5663)(12.3830, 8.6217)(14.8600, 8.6872)(17.8320, 8.7133)(21.3980, 8.7767)(25.6780, 8.7900)(30.8140, 8.8326)(36.9760, 8.8480)
        };  \addlegendentry {$B$ = 10}

        \addplot[color=red, mark=o, width = \plotwidth] coordinates {
            (2.0000, 7.8602)(2.4000, 7.8214)(2.8800, 7.7878)(3.4550, 7.7147)(4.1470, 7.6802)(4.9760, 8.0632)(5.9710, 8.1357)(7.1660, 8.1716)(8.5990, 8.2139)(10.3190, 8.2648)(12.3830, 8.3040)(14.8600, 8.3567)(17.8320, 8.3857)(21.3980, 8.4610)(25.6780, 8.5049)(30.8140, 8.5687)(36.9760, 8.6228)
        };  \addlegendentry {$B$ = 30}
        
        \addplot[color=blue, mark=x, width = \plotwidth]    coordinates {
            (2.0000, 7.8602)(2.4000, 7.8214)(2.8800, 7.7878)(3.4550, 7.7147)(4.1470, 7.6802)(4.9760, 7.6414)(5.9710, 7.6151)(7.1660, 7.5981)(8.5990, 8.0830)(10.3190, 8.1277)(12.3830, 8.1676)(14.8600, 8.2125)(17.8320, 8.2644)(21.3980, 8.3044)(25.6780, 8.3566)(30.8140, 8.3857)(36.9760, 8.4610)
        };  \addlegendentry {$B$ = 50}



        \end{axis}
        \end{tikzpicture}
    }
    
        \subfloat [ C=1000 Lfu $\missp = 10$ Scarab] { 
        \begin{tikzpicture}
        	\begin{axis}[
        		width  = \plotwidth,
         		height = \plotheight,
        		xmin = \xmin,
        		xmax = \xmax,
        		legend style = {at={(0.5,1.23)},anchor=north,legend columns=-1,font=\footnotesize},
        		ylabel = Service Cost,
         		ylabel near ticks,
        		xlabel = {Indicator Size [bits per element]},
        		xlabel near ticks,
        	    label style={font=\footnotesize},
        	    tick label style={font=\footnotesize},
        	]
        \addplot[color=black, mark=triangle, width = \plotwidth] coordinates {
            (2.0000, 7.3329)(2.4000, 7.3548)(2.8800, 7.3371)(3.4550, 7.3181)(4.1470, 7.3013)(4.9760, 7.2911)(5.9710, 7.2786)(7.1660, 7.2721)(8.5990, 7.2777)(10.3190, 7.2837)(12.3830, 7.2891)(14.8600, 7.3006)(17.8320, 7.3186)(21.3980, 7.3355)(25.6780, 7.3581)(30.8140, 7.3702)(36.9760, 7.3904)
        };  \addlegendentry {$B$ = 10}
        
        \addplot[color=red, mark=o, width = \plotwidth] coordinates {
            (2.0000, 7.3329)(2.4000, 7.2975)(2.8800, 7.2662)(3.4550, 7.1979)(4.1470, 7.1652)(4.9760, 7.1319)(5.9710, 7.2155)(7.1660, 7.2117)(8.5990, 7.2260)(10.3190, 7.2300)(12.3830, 7.2364)(14.8600, 7.2501)(17.8320, 7.2566)(21.3980, 7.2628)(25.6780, 7.2740)(30.8140, 7.2804)(36.9760, 7.3003)
        };  \addlegendentry {$B$ = 30}
        
        \addplot[color=blue, mark=x, width = \plotwidth]    coordinates {
            (2.0000, 7.3329)(2.4000, 7.2975)(2.8800, 7.2662)(3.4550, 7.1979)(4.1470, 7.1652)(4.9760, 7.1319)(5.9710, 7.1061)(7.1660, 7.0894)(8.5990, 7.1644)(10.3190, 7.1981)(12.3830, 7.2074)(14.8600, 7.2177)(17.8320, 7.2352)(21.3980, 7.2428)(25.6780, 7.2496)(30.8140, 7.2564)(36.9760, 7.2699)
        };  \addlegendentry {$B$ = 50}

        \end{axis}
    \end{tikzpicture}
    }
    
    \subfloat [ C=10,000 Lru $\missp = 3$ Scarab] { 
        \begin{tikzpicture}
        	\begin{axis}[
        		width  = \plotwidth,
         		height = \plotheight,
        		xmin = \xmin,
        		xmax = \xmax,
        		legend style = {at={(0.5,1.23)},anchor=north,legend columns=-1,font=\footnotesize},
        		ylabel = Service Cost,
         		ylabel near ticks,
        		xlabel = {Indicator Size [bits per element]},
        		xlabel near ticks,
        	    label style={font=\footnotesize},
        	    tick label style={font=\footnotesize},
        	]
\addplot[color=black, mark=triangle, width = \plotwidth] coordinates {
(2.0000, 2.2272)(2.4000, 2.2738)(2.8800, 2.2878)(3.4559, 2.2643)(4.1472, 2.2557)(4.9766, 2.2461)(5.9719, 2.2445)(7.1663, 2.2497)(8.5996, 2.2585)(10.3195, 2.2701)(12.3834, 2.2872)(14.8601, 2.3075)(17.8322, 2.3286)(21.3986, 2.3286)(25.6783, 2.3549)(30.8140, 2.3549)(36.9768, 2.3818)
};  \addlegendentry {$B$ = 10}

\addplot[color=red, mark=o, width = \plotwidth] coordinates {
(2.0000, 2.2272)(2.4000, 2.2008)(2.8800, 2.1759)(3.4559, 2.1254)(4.1472, 2.1015)(4.9766, 2.0742)(5.9719, 2.1919)(7.1663, 2.1960)(8.5996, 2.1976)(10.3195, 2.2019)(12.3834, 2.2083)(14.8601, 2.2169)(17.8322, 2.2270)(21.3986, 2.2398)(25.6783, 2.2537)(30.8140, 2.2682)(36.9768, 2.2682)
};  \addlegendentry {$B$ = 30}

\addplot[color=blue, mark=x, width = \plotwidth]    coordinates {
(2.0000, 2.2272)(2.4000, 2.2008)(2.8800, 2.1759)(3.4559, 2.1254)(4.1472, 2.1015)(4.9766, 2.0742)(5.9719, 2.0560)(7.1663, 2.0440)(8.5996, 2.0355)(10.3195, 2.1811)(12.3834, 2.1853)(14.8601, 2.1921)(17.8322, 2.1996)(21.3986, 2.2074)(25.6783, 2.2165)(30.8140, 2.2269)(36.9768, 2.2398)
};  \addlegendentry {$B$ = 50}

        \end{axis}
    \end{tikzpicture}
    }
    
        \subfloat [ C=10,000 Lru M10 Scarab] { 
        \begin{tikzpicture}
        	\begin{axis}[
        		width  = \plotwidth,
         		height = \plotheight,
        		xmin = \xmin,
        		xmax = \xmax,
        		legend style = {at={(0.5,1.23)},anchor=north,legend columns=-1,font=\footnotesize},
        		ylabel = Service Cost,
         		ylabel near ticks,
        		xlabel = {Indicator Size [bits per element]},
        		xlabel near ticks,
        	    label style={font=\footnotesize},
        	    tick label style={font=\footnotesize},
        	]
\addplot[color=black, mark=triangle, width = \plotwidth] coordinates {
(2.0000, 5.8220)(2.4000, 6.1198)(2.8800, 6.2551)(3.4559, 6.3140)(4.1472, 6.3499)(4.9766, 6.3914)(5.9719, 6.4364)(7.1663, 6.4896)(8.5996, 6.5433)(10.3195, 6.5994)(12.3834, 6.6633)(14.8601, 6.7383)(17.8322, 6.8187)(21.3986, 6.8190)(25.6783, 6.9136)(30.8140, 6.9136)(36.9768, 7.0218)
};  \addlegendentry {$B$ = 10}

\addplot[color=red, mark=o, width = \plotwidth] coordinates {
(2.0000, 5.8220)(2.4000, 5.7956)(2.8800, 5.7707)(3.4559, 5.7202)(4.1472, 5.6963)(4.9766, 5.6691)(5.9719, 6.2432)(7.1663, 6.2956)(8.5996, 6.3251)(10.3195, 6.3562)(12.3834, 6.3849)(14.8601, 6.4180)(17.8322, 6.4545)(21.3986, 6.5012)(25.6783, 6.5494)(30.8140, 6.6026)(36.9768, 6.6026)
};  \addlegendentry {$B$ = 30}

\addplot[color=blue, mark=x, width = \plotwidth]    coordinates {
(2.0000, 5.8220)(2.4000, 5.7956)(2.8800, 5.7707)(3.4559, 5.7202)(4.1472, 5.6963)(4.9766, 5.6691)(5.9719, 5.6508)(7.1663, 5.6389)(8.5996, 5.6304)(10.3195, 6.2780)(12.3834, 6.3006)(14.8601, 6.3281)(17.8322, 6.3577)(21.3986, 6.3853)(25.6783, 6.4179)(30.8140, 6.4545)(36.9768, 6.5013)
};  \addlegendentry {$B$ = 50}

        \end{axis}
    \end{tikzpicture}
    }
\end{figure}
\begin{figure}    
    \subfloat [ C1K Lfu $\missp = 3$ Gradle] { 
        \begin{tikzpicture}
        	\begin{axis}[
        		width  = \plotwidth,
         		height = \plotheight,
        		xmin = \xmin,
        		xmax = \xmax,
        		legend style = {at={(0.5,1.23)},anchor=north,legend columns=-1,font=\footnotesize},
        		ylabel = Service Cost,
         		ylabel near ticks,
        		xlabel = {Indicator Size [bits per element]},
        		xlabel near ticks,
        	    label style={font=\footnotesize},
        	    tick label style={font=\footnotesize},
        	]
\addplot[color=black, mark=triangle, width = \plotwidth] coordinates {
(2.0000, 1.6133)(2.4000, 1.5998)(2.8800, 1.5883)(3.4550, 1.5620)(4.1470, 1.5498)(4.9760, 1.5487)(5.9710, 1.5453)(7.1660, 1.5422)(8.5990, 1.5446)(10.3190, 1.5474)(12.3830, 1.5521)(14.8600, 1.5587)
};  \addlegendentry {$B$ = 10}

\addplot[color=red, mark=o, width = \plotwidth] coordinates {
(2.0000, 1.6133)(2.4000, 1.5998)(2.8800, 1.5883)(3.4550, 1.5620)(4.1470, 1.5498)(4.9760, 1.5363)(5.9710, 1.5268)(7.1660, 1.5213)(8.5990, 1.5167)(10.3190, 1.5142)(12.3830, 1.5154)(14.8600, 1.5301)
};  \addlegendentry {$B$ = 30}

\addplot[color=blue, mark=x, width = \plotwidth]    coordinates {
(2.0000, 1.6133)(2.4000, 1.5998)(2.8800, 1.5883)(3.4550, 1.5620)(4.1470, 1.5498)(4.9760, 1.5363)(5.9710, 1.5268)(7.1660, 1.5213)(8.5990, 1.5167)(10.3190, 1.5142)(12.3830, 1.5131)(14.8600, 1.5126)
};  \addlegendentry {$B$ = 50}

        \end{axis}
    \end{tikzpicture}
    }
    
        \subfloat [ C1K Lfu $\missp = 10$ Gradle] { 
        \begin{tikzpicture}
        	\begin{axis}[
        		width  = \plotwidth,
         		height = \plotheight,
        		xmin = \xmin,
        		xmax = \xmax,
        		legend style = {at={(0.5,1.23)},anchor=north,legend columns=-1,font=\footnotesize},
        		ylabel = Service Cost,
         		ylabel near ticks,
        		xlabel = {Indicator Size [bits per element]},
        		xlabel near ticks,
        	    label style={font=\footnotesize},
        	    tick label style={font=\footnotesize},
        	]
\addplot[color=black, mark=triangle, width = \plotwidth] coordinates {
(2.0000, 3.4067)(2.4000, 3.3932)(2.8800, 3.3817)(3.4550, 3.3553)(4.1470, 3.3431)(4.9760, 3.3753)(5.9710, 3.3881)(7.1660, 3.3916)(8.5990, 3.4142)(10.3190, 3.4341)(12.3830, 3.4577)(14.8600, 3.4886)
};  \addlegendentry {$B$ = 10}

\addplot[color=red, mark=o, width = \plotwidth] coordinates {
(2.0000, 3.4067)(2.4000, 3.3932)(2.8800, 3.3817)(3.4550, 3.3553)(4.1470, 3.3431)(4.9760, 3.3296)(5.9710, 3.3202)(7.1660, 3.3146)(8.5990, 3.3100)(10.3190, 3.3075)(12.3830, 3.3151)(14.8600, 3.3697)
};  \addlegendentry {$B$ = 30}

\addplot[color=blue, mark=x, width = \plotwidth]    coordinates {
(2.0000, 3.4067)(2.4000, 3.3932)(2.8800, 3.3817)(3.4550, 3.3553)(4.1470, 3.3431)(4.9760, 3.3296)(5.9710, 3.3202)(7.1660, 3.3146)(8.5990, 3.3100)(10.3190, 3.3075)(12.3830, 3.3064)(14.8600, 3.3060)
};  \addlegendentry {$B$ = 50}


        \end{axis}
    \end{tikzpicture}
    }
\end{figure}


==> traces.tex <==
\section{Evaluation}
\subsection{Traces}
\gabi{give references to traces source}
\paragraph{Scarab}
A one-hour trace from Scarab Research, a personalized recommendation system for e-commerce sites.

\paragraph{Gradle}
Gradle is a build tool that extensively use caching, so that subsequent builds on different machines fetch parts of the build tree that are cached and up to date, instead of re-building. Due to the importance of the requested data being the most updated, this trace is recency-biased. 
This trace was provided by the Gradle project.

\paragraph{WS}
~\cite{Umass_traces}

\paragraph{F}
~\cite{Umass_traces}

